CO$_2$ and NO$_2$ Formation on Amorphous Solid Water

The dynamics for molecule formation, relaxation, diffusion, and desorption on amorphous solid water is studied in a quantitative fashion. We aim at characterizing, at a quantitative level, the formation probability, stabilization, energy relaxation and diffusion dynamics of CO$_2$ and NO$_2$ on cold amorphous solid water following atom+diatom recombination reactions. Accurate machine-learned energy functions combined with fluctuating charge models were used to investigate the diffusion, interactions, and recombination dynamics of atomic oxygen with CO and NO on amorphous solid water (ASW). Energy relaxation to the ASW and into water-internal-degrees of freedom were determined from analysis of the vibrational density of states. The surface diffusion and desorption energetics was investigated from extended and nonequilibrium MD simulations. The reaction probability on the nanosecond time scale is determined in a quantitative fashion and demonstrates that surface diffusion of the reactants leads to recombination for initial separations up to 20 \AA\/. After recombination both, CO$_2$ and NO$_2$, stabilize by energy transfer to water internal and surface phonon modes on the picosecond time scale. The average diffusion barriers and desorption energies agree with those reported from experiments. After recombination, the triatomic products diffuse easily which contrasts with the equilibrium situation in which both, CO$_2$ and NO$_2$, are stationary on the multi-nanosecond time scale.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

